A Fast Octree-Based Algorithm for Computing Ropelength

The ropelength of a space curve is usually defined as the quotient of its length by its thickness: the radius of the largest embedded tube around the knot. This idea was extended to space polygons by Eric Rawdon, who gave a definition of ropelength in terms of doubly-critical self-distances (local minima of the distance function on pairs of points on the polygon) and a function of the exterior angles of the polygon. A naive algorithm for finding the doubly-critical self-distances of an n-edge polygon involves comparing each pair of edges, and so takes O(n^2) time. In this paper, we describe an improved algorithm, based on the notion of octrees, which runs in O(n log n) time. The speed of the ropelength computation controls the performance of ropelength-minimizing programs such as Rawdon and Piatek's TOROS. An implementation of our algorithm is freely available under the GNU Public License.

==> figs/trefoil_logplot.tex <==
% GNUPLOT: LaTeX picture using EEPIC macros
\setlength{\unitlength}{0.120450pt}
\begin{picture}(3000,1800)(0,0)
\footnotesize
\thicklines \path(410,166)(451,166)
\thicklines \path(2876,166)(2835,166)
\put(369,166){\makebox(0,0)[r]{ 0.0001}}
\thicklines \path(410,233)(430,233)
\thicklines \path(2876,233)(2856,233)
\thicklines \path(410,321)(430,321)
\thicklines \path(2876,321)(2856,321)
\thicklines \path(410,366)(430,366)
\thicklines \path(2876,366)(2856,366)
\thicklines \path(410,388)(451,388)
\thicklines \path(2876,388)(2835,388)
\put(369,388){\makebox(0,0)[r]{ 0.001}}
\thicklines \path(410,454)(430,454)
\thicklines \path(2876,454)(2856,454)
\thicklines \path(410,543)(430,543)
\thicklines \path(2876,543)(2856,543)
\thicklines \path(410,588)(430,588)
\thicklines \path(2876,588)(2856,588)
\thicklines \path(410,609)(451,609)
\thicklines \path(2876,609)(2835,609)
\put(369,609){\makebox(0,0)[r]{ 0.01}}
\thicklines \path(410,676)(430,676)
\thicklines \path(2876,676)(2856,676)
\thicklines \path(410,764)(430,764)
\thicklines \path(2876,764)(2856,764)
\thicklines \path(410,810)(430,810)
\thicklines \path(2876,810)(2856,810)
\thicklines \path(410,831)(451,831)
\thicklines \path(2876,831)(2835,831)
\put(369,831){\makebox(0,0)[r]{ 0.1}}
\thicklines \path(410,898)(430,898)
\thicklines \path(2876,898)(2856,898)
\thicklines \path(410,986)(430,986)
\thicklines \path(2876,986)(2856,986)
\thicklines \path(410,1031)(430,1031)
\thicklines \path(2876,1031)(2856,1031)
\thicklines \path(410,1053)(451,1053)
\thicklines \path(2876,1053)(2835,1053)
\put(369,1053){\makebox(0,0)[r]{ 1}}
\thicklines \path(410,1120)(430,1120)
\thicklines \path(2876,1120)(2856,1120)
\thicklines \path(410,1208)(430,1208)
\thicklines \path(2876,1208)(2856,1208)
\thicklines \path(410,1253)(430,1253)
\thicklines \path(2876,1253)(2856,1253)
\thicklines \path(410,1275)(451,1275)
\thicklines \path(2876,1275)(2835,1275)
\put(369,1275){\makebox(0,0)[r]{ 10}}
\thicklines \path(410,1341)(430,1341)
\thicklines \path(2876,1341)(2856,1341)
\thicklines \path(410,1430)(430,1430)
\thicklines \path(2876,1430)(2856,1430)
\thicklines \path(410,1475)(430,1475)
\thicklines \path(2876,1475)(2856,1475)
\thicklines \path(410,1496)(451,1496)
\thicklines \path(2876,1496)(2835,1496)
\put(369,1496){\makebox(0,0)[r]{ 100}}
\thicklines \path(410,1563)(430,1563)
\thicklines \path(2876,1563)(2856,1563)
\thicklines \path(410,1651)(430,1651)
\thicklines \path(2876,1651)(2856,1651)
\thicklines \path(410,1697)(430,1697)
\thicklines \path(2876,1697)(2856,1697)
\thicklines \path(410,1718)(451,1718)
\thicklines \path(2876,1718)(2835,1718)
\put(369,1718){\makebox(0,0)[r]{ 1000}}
\thicklines \path(410,166)(410,207)
\thicklines \path(410,1718)(410,1677)
\put(410,83){\makebox(0,0){ 10}}
\thicklines \path(596,166)(596,186)
\thicklines \path(596,1718)(596,1698)
\thicklines \path(704,166)(704,186)
\thicklines \path(704,1718)(704,1698)
\thicklines \path(781,166)(781,186)
\thicklines \path(781,1718)(781,1698)
\thicklines \path(841,166)(841,186)
\thicklines \path(841,1718)(841,1698)
\thicklines \path(890,166)(890,186)
\thicklines \path(890,1718)(890,1698)
\thicklines \path(931,166)(931,186)
\thicklines \path(931,1718)(931,1698)
\thicklines \path(967,166)(967,186)
\thicklines \path(967,1718)(967,1698)
\thicklines \path(998,166)(998,186)
\thicklines \path(998,1718)(998,1698)
\thicklines \path(1027,166)(1027,207)
\thicklines \path(1027,1718)(1027,1677)
\put(1027,83){\makebox(0,0){ 100}}
\thicklines \path(1212,166)(1212,186)
\thicklines \path(1212,1718)(1212,1698)
\thicklines \path(1321,166)(1321,186)
\thicklines \path(1321,1718)(1321,1698)
\thicklines \path(1398,166)(1398,186)
\thicklines \path(1398,1718)(1398,1698)
\thicklines \path(1457,166)(1457,186)
\thicklines \path(1457,1718)(1457,1698)
\thicklines \path(1506,166)(1506,186)
\thicklines \path(1506,1718)(1506,1698)
\thicklines \path(1548,166)(1548,186)
\thicklines \path(1548,1718)(1548,1698)
\thicklines \path(1583,166)(1583,186)
\thicklines \path(1583,1718)(1583,1698)
\thicklines \path(1615,166)(1615,186)
\thicklines \path(1615,1718)(1615,1698)
\thicklines \path(1643,166)(1643,207)
\thicklines \path(1643,1718)(1643,1677)
\put(1643,83){\makebox(0,0){ 1000}}
\thicklines \path(1829,166)(1829,186)
\thicklines \path(1829,1718)(1829,1698)
\thicklines \path(1937,166)(1937,186)
\thicklines \path(1937,1718)(1937,1698)
\thicklines \path(2014,166)(2014,186)
\thicklines \path(2014,1718)(2014,1698)
\thicklines \path(2074,166)(2074,186)
\thicklines \path(2074,1718)(2074,1698)
\thicklines \path(2123,166)(2123,186)
\thicklines \path(2123,1718)(2123,1698)
\thicklines \path(2164,166)(2164,186)
\thicklines \path(2164,1718)(2164,1698)
\thicklines \path(2200,166)(2200,186)
\thicklines \path(2200,1718)(2200,1698)
\thicklines \path(2231,166)(2231,186)
\thicklines \path(2231,1718)(2231,1698)
\thicklines \path(2260,166)(2260,207)
\thicklines \path(2260,1718)(2260,1677)
\put(2260,83){\makebox(0,0){ 10000}}
\thicklines \path(2445,166)(2445,186)
\thicklines \path(2445,1718)(2445,1698)
\thicklines \path(2554,166)(2554,186)
\thicklines \path(2554,1718)(2554,1698)
\thicklines \path(2631,166)(2631,186)
\thicklines \path(2631,1718)(2631,1698)
\thicklines \path(2690,166)(2690,186)
\thicklines \path(2690,1718)(2690,1698)
\thicklines \path(2739,166)(2739,186)
\thicklines \path(2739,1718)(2739,1698)
\thicklines \path(2781,166)(2781,186)
\thicklines \path(2781,1718)(2781,1698)
\thicklines \path(2816,166)(2816,186)
\thicklines \path(2816,1718)(2816,1698)
\thicklines \path(2848,166)(2848,186)
\thicklines \path(2848,1718)(2848,1698)
\thicklines \path(2876,166)(2876,207)
\thicklines \path(2876,1718)(2876,1677)
\put(2876,83){\makebox(0,0){ 100000}}
\thicklines \path(410,166)(2876,166)(2876,1718)(410,1718)(410,166)
\put(2548,1636){\makebox(0,0)[r]{'trefoil_fast.dat'}}
\thinlines \path(2589,1636)(2794,1636)
\thinlines \path(410,166)(410,166)(596,233)(704,321)(781,388)(841,405)(890,433)(931,464)(967,480)(998,500)(1027,506)(1052,511)(1075,524)(1097,535)(1117,539)(1135,550)(1152,541)(1169,560)(1184,575)(1198,563)(1212,582)(1225,563)(1238,579)(1250,597)(1261,607)(1272,593)(1282,619)(1292,627)(1302,632)(1312,639)(1321,640)(1329,619)(1338,624)(1346,651)(1354,654)(1362,659)(1369,662)(1377,656)(1384,642)(1391,668)(1398,673)(1404,677)(1411,682)(1417,685)(1423,656)(1429,684)(1435,688)(1441,693)(1446,695)(1452,698)(1457,671)
\thinlines \path(1457,671)(1457,671)(1506,735)(1548,748)(1583,760)(1615,772)(1643,756)(1669,805)(1692,823)(1713,824)(1733,837)(1752,813)(1769,849)(1785,864)(1800,864)(1815,873)(1829,844)(1937,890)(2014,922)(2074,951)(2123,979)(2164,997)(2200,1014)(2231,1032)(2260,1043)(2285,1055)(2308,1065)(2330,1074)(2350,1084)(2368,1093)(2385,1101)(2402,1102)(2417,1116)(2431,1114)(2445,1128)
\put(410,166){\circle{12}}
\put(596,233){\circle{12}}
\put(704,321){\circle{12}}
\put(781,388){\circle{12}}
\put(841,405){\circle{12}}
\put(890,433){\circle{12}}
\put(931,464){\circle{12}}
\put(967,480){\circle{12}}
\put(998,500){\circle{12}}
\put(1027,506){\circle{12}}
\put(1052,511){\circle{12}}
\put(1075,524){\circle{12}}
\put(1097,535){\circle{12}}
\put(1117,539){\circle{12}}
\put(1135,550){\circle{12}}
\put(1152,541){\circle{12}}
\put(1169,560){\circle{12}}
\put(1184,575){\circle{12}}
\put(1198,563){\circle{12}}
\put(1212,582){\circle{12}}
\put(1225,563){\circle{12}}
\put(1238,579){\circle{12}}
\put(1250,597){\circle{12}}
\put(1261,607){\circle{12}}
\put(1272,593){\circle{12}}
\put(1282,619){\circle{12}}
\put(1292,627){\circle{12}}
\put(1302,632){\circle{12}}
\put(1312,639){\circle{12}}
\put(1321,640){\circle{12}}
\put(1329,619){\circle{12}}
\put(1338,624){\circle{12}}
\put(1346,651){\circle{12}}
\put(1354,654){\circle{12}}
\put(1362,659){\circle{12}}
\put(1369,662){\circle{12}}
\put(1377,656){\circle{12}}
\put(1384,642){\circle{12}}
\put(1391,668){\circle{12}}
\put(1398,673){\circle{12}}
\put(1404,677){\circle{12}}
\put(1411,682){\circle{12}}
\put(1417,685){\circle{12}}
\put(1423,656){\circle{12}}
\put(1429,684){\circle{12}}
\put(1435,688){\circle{12}}
\put(1441,693){\circle{12}}
\put(1446,695){\circle{12}}
\put(1452,698){\circle{12}}
\put(1457,671){\circle{12}}
\put(1457,671){\circle{12}}
\put(1506,735){\circle{12}}
\put(1548,748){\circle{12}}
\put(1583,760){\circle{12}}
\put(1615,772){\circle{12}}
\put(1643,756){\circle{12}}
\put(1669,805){\circle{12}}
\put(1692,823){\circle{12}}
\put(1713,824){\circle{12}}
\put(1733,837){\circle{12}}
\put(1752,813){\circle{12}}
\put(1769,849){\circle{12}}
\put(1785,864){\circle{12}}
\put(1800,864){\circle{12}}
\put(1815,873){\circle{12}}
\put(1829,844){\circle{12}}
\put(1937,890){\circle{12}}
\put(2014,922){\circle{12}}
\put(2074,951){\circle{12}}
\put(2123,979){\circle{12}}
\put(2164,997){\circle{12}}
\put(2200,1014){\circle{12}}
\put(2231,1032){\circle{12}}
\put(2260,1043){\circle{12}}
\put(2285,1055){\circle{12}}
\put(2308,1065){\circle{12}}
\put(2330,1074){\circle{12}}
\put(2350,1084){\circle{12}}
\put(2368,1093){\circle{12}}
\put(2385,1101){\circle{12}}
\put(2402,1102){\circle{12}}
\put(2417,1116){\circle{12}}
\put(2431,1114){\circle{12}}
\put(2445,1128){\circle{12}}
\put(2691,1636){\circle{12}}
\put(2548,1553){\makebox(0,0)[r]{'trefoil_slow.dat'}}
\thicklines \path(2589,1553)(2794,1553)
\thicklines \path(410,166)(410,166)(596,166)(704,272)(781,299)(841,366)(890,388)(931,420)(967,444)(998,468)(1027,487)(1052,506)(1075,524)(1097,537)(1117,550)(1135,563)(1152,576)(1169,587)(1184,598)(1198,608)(1212,619)(1225,627)(1238,637)(1250,645)(1261,653)(1272,662)(1282,669)(1292,676)(1302,684)(1312,689)(1321,697)(1329,702)(1338,709)(1346,715)(1354,720)(1362,725)(1369,732)(1377,736)(1384,742)(1391,746)(1398,752)(1404,756)(1411,760)(1417,765)(1423,769)(1429,775)(1435,778)(1441,783)(1446,786)(1452,792)(1457,794)
\thicklines \path(1457,794)(1457,794)(1506,830)(1548,861)(1583,886)(1615,909)(1643,930)(1669,947)(1692,964)(1713,980)(1733,994)(1752,1008)(1769,1020)(1785,1032)(1800,1043)(1815,1054)(1829,1063)(1937,1145)(2014,1209)(2074,1266)(2123,1311)(2164,1346)(2200,1373)(2231,1396)(2260,1417)(2285,1436)(2308,1453)(2330,1468)(2350,1483)(2368,1496)(2385,1509)(2402,1521)(2417,1532)(2431,1543)(2445,1553)
\put(410,166){\makebox(0,0){$\star$}}
\put(596,166){\makebox(0,0){$\star$}}
\put(704,272){\makebox(0,0){$\star$}}
\put(781,299){\makebox(0,0){$\star$}}
\put(841,366){\makebox(0,0){$\star$}}
\put(890,388){\makebox(0,0){$\star$}}
\put(931,420){\makebox(0,0){$\star$}}
\put(967,444){\makebox(0,0){$\star$}}
\put(998,468){\makebox(0,0){$\star$}}
\put(1027,487){\makebox(0,0){$\star$}}
\put(1052,506){\makebox(0,0){$\star$}}
\put(1075,524){\makebox(0,0){$\star$}}
\put(1097,537){\makebox(0,0){$\star$}}
\put(1117,550){\makebox(0,0){$\star$}}
\put(1135,563){\makebox(0,0){$\star$}}
\put(1152,576){\makebox(0,0){$\star$}}
\put(1169,587){\makebox(0,0){$\star$}}
\put(1184,598){\makebox(0,0){$\star$}}
\put(1198,608){\makebox(0,0){$\star$}}
\put(1212,619){\makebox(0,0){$\star$}}
\put(1225,627){\makebox(0,0){$\star$}}
\put(1238,637){\makebox(0,0){$\star$}}
\put(1250,645){\makebox(0,0){$\star$}}
\put(1261,653){\makebox(0,0){$\star$}}
\put(1272,662){\makebox(0,0){$\star$}}
\put(1282,669){\makebox(0,0){$\star$}}
\put(1292,676){\makebox(0,0){$\star$}}
\put(1302,684){\makebox(0,0){$\star$}}
\put(1312,689){\makebox(0,0){$\star$}}
\put(1321,697){\makebox(0,0){$\star$}}
\put(1329,702){\makebox(0,0){$\star$}}
\put(1338,709){\makebox(0,0){$\star$}}
\put(1346,715){\makebox(0,0){$\star$}}
\put(1354,720){\makebox(0,0){$\star$}}
\put(1362,725){\makebox(0,0){$\star$}}
\put(1369,732){\makebox(0,0){$\star$}}
\put(1377,736){\makebox(0,0){$\star$}}
\put(1384,742){\makebox(0,0){$\star$}}
\put(1391,746){\makebox(0,0){$\star$}}
\put(1398,752){\makebox(0,0){$\star$}}
\put(1404,756){\makebox(0,0){$\star$}}
\put(1411,760){\makebox(0,0){$\star$}}
\put(1417,765){\makebox(0,0){$\star$}}
\put(1423,769){\makebox(0,0){$\star$}}
\put(1429,775){\makebox(0,0){$\star$}}
\put(1435,778){\makebox(0,0){$\star$}}
\put(1441,783){\makebox(0,0){$\star$}}
\put(1446,786){\makebox(0,0){$\star$}}
\put(1452,792){\makebox(0,0){$\star$}}
\put(1457,794){\makebox(0,0){$\star$}}
\put(1457,794){\makebox(0,0){$\star$}}
\put(1506,830){\makebox(0,0){$\star$}}
\put(1548,861){\makebox(0,0){$\star$}}
\put(1583,886){\makebox(0,0){$\star$}}
\put(1615,909){\makebox(0,0){$\star$}}
\put(1643,930){\makebox(0,0){$\star$}}
\put(1669,947){\makebox(0,0){$\star$}}
\put(1692,964){\makebox(0,0){$\star$}}
\put(1713,980){\makebox(0,0){$\star$}}
\put(1733,994){\makebox(0,0){$\star$}}
\put(1752,1008){\makebox(0,0){$\star$}}
\put(1769,1020){\makebox(0,0){$\star$}}
\put(1785,1032){\makebox(0,0){$\star$}}
\put(1800,1043){\makebox(0,0){$\star$}}
\put(1815,1054){\makebox(0,0){$\star$}}
\put(1829,1063){\makebox(0,0){$\star$}}
\put(1937,1145){\makebox(0,0){$\star$}}
\put(2014,1209){\makebox(0,0){$\star$}}
\put(2074,1266){\makebox(0,0){$\star$}}
\put(2123,1311){\makebox(0,0){$\star$}}
\put(2164,1346){\makebox(0,0){$\star$}}
\put(2200,1373){\makebox(0,0){$\star$}}
\put(2231,1396){\makebox(0,0){$\star$}}
\put(2260,1417){\makebox(0,0){$\star$}}
\put(2285,1436){\makebox(0,0){$\star$}}
\put(2308,1453){\makebox(0,0){$\star$}}
\put(2330,1468){\makebox(0,0){$\star$}}
\put(2350,1483){\makebox(0,0){$\star$}}
\put(2368,1496){\makebox(0,0){$\star$}}
\put(2385,1509){\makebox(0,0){$\star$}}
\put(2402,1521){\makebox(0,0){$\star$}}
\put(2417,1532){\makebox(0,0){$\star$}}
\put(2431,1543){\makebox(0,0){$\star$}}
\put(2445,1553){\makebox(0,0){$\star$}}
\put(2691,1553){\makebox(0,0){$\star$}}
\thicklines \path(410,166)(2876,166)(2876,1718)(410,1718)(410,166)
\end{picture}

